Radiative correction on moduli stabilization in modular flavor symmetric models

We study the radiative corrections to the stabilization of the complex structure modulus $\tau$ in modular flavor symmetric models. We discuss the possibility of obtaining the vacuum expectation value of $\tau$ in the vicinity of the fixed point where residual symmetries remain unbroken. As concrete examples, we analyze the 1-loop Coleman-Weinberg potential in the $A_4$ modular flavor models. We show that the 1-loop correction may lead to the slight deviation from the tree level result, which may realize a phenomenologically preferred value of the complex structure modulus $\tau$ particularly when the number of species contributing to the 1-loop correction is large enough.

==> main-references.tex <==
%\cite{Feruglio:2017spp}
\bibitem{Feruglio:2017spp}
F.~Feruglio,
%``Are neutrino masses modular forms?,''
doi:10.1142/9789813238053\_0012
[arXiv:1706.08749 [hep-ph]].
%214 citations counted in INSPIRE as of 17 Oct 2023

%\cite{Kobayashi:2018vbk}
\bibitem{Kobayashi:2018vbk}
T.~Kobayashi, K.~Tanaka and T.~H.~Tatsuishi,
%``Neutrino mixing from finite modular groups,''
Phys. Rev. D \textbf{98}, no.1, 016004 (2018)
doi:10.1103/PhysRevD.98.016004
[arXiv:1803.10391 [hep-ph]].
%179 citations counted in INSPIRE as of 17 Oct 2023

%\cite{Penedo:2018nmg}
\bibitem{Penedo:2018nmg}
J.~T.~Penedo and S.~T.~Petcov,
%``Lepton Masses and Mixing from Modular $S_4$ Symmetry,''
Nucl. Phys. B \textbf{939}, 292-307 (2019)
doi:10.1016/j.nuclphysb.2018.12.016
[arXiv:1806.11040 [hep-ph]].
%179 citations counted in INSPIRE as of 17 Oct 2023

%\cite{Criado:2018thu}
\bibitem{Criado:2018thu}
J.~C.~Criado and F.~Feruglio,
%``Modular Invariance Faces Precision Neutrino Data,''
SciPost Phys. \textbf{5}, no.5, 042 (2018)
doi:10.21468/SciPostPhys.5.5.042
[arXiv:1807.01125 [hep-ph]].
%178 citations counted in INSPIRE as of 17 Oct 2023

%\cite{Kobayashi:2018scp}
\bibitem{Kobayashi:2018scp}
T.~Kobayashi, N.~Omoto, Y.~Shimizu, K.~Takagi, M.~Tanimoto and T.~H.~Tatsuishi,
%``Modular A$_{4}$ invariance and neutrino mixing,''
JHEP \textbf{11}, 196 (2018)
doi:10.1007/JHEP11(2018)196
[arXiv:1808.03012 [hep-ph]].
%166 citations counted in INSPIRE as of 17 Oct 2023

%\cite{Novichkov:2018ovf}
\bibitem{Novichkov:2018ovf}
P.~P.~Novichkov, J.~T.~Penedo, S.~T.~Petcov and A.~V.~Titov,
%``Modular S$_{4}$ models of lepton masses and mixing,''
JHEP \textbf{04}, 005 (2019)
doi:10.1007/JHEP04(2019)005
[arXiv:1811.04933 [hep-ph]].
%170 citations counted in INSPIRE as of 17 Oct 2023

%\cite{Novichkov:2018nkm}
\bibitem{Novichkov:2018nkm}
P.~P.~Novichkov, J.~T.~Penedo, S.~T.~Petcov and A.~V.~Titov,
%``Modular A$_{5}$ symmetry for flavour model building,''
JHEP \textbf{04}, 174 (2019)
doi:10.1007/JHEP04(2019)174
[arXiv:1812.02158 [hep-ph]].
%162 citations counted in INSPIRE as of 17 Oct 2023

%\cite{deAnda:2018ecu}
\bibitem{deAnda:2018ecu}
F.~J.~de Anda, S.~F.~King and E.~Perdomo,
%``$SU(5)$ grand unified theory with $A_4$ modular symmetry,''
Phys. Rev. D \textbf{101}, no.1, 015028 (2020)
doi:10.1103/PhysRevD.101.015028
[arXiv:1812.05620 [hep-ph]].
%143 citations counted in INSPIRE as of 17 Oct 2023

%\cite{Okada:2018yrn}
\bibitem{Okada:2018yrn}
H.~Okada and M.~Tanimoto,
%``CP violation of quarks in $A_4$ modular invariance,''
Phys. Lett. B \textbf{791}, 54-61 (2019)
doi:10.1016/j.physletb.2019.02.028
[arXiv:1812.09677 [hep-ph]].
%143 citations counted in INSPIRE as of 17 Oct 2023

%\cite{Kobayashi:2018wkl}
\bibitem{Kobayashi:2018wkl}
T.~Kobayashi, Y.~Shimizu, K.~Takagi, M.~Tanimoto, T.~H.~Tatsuishi and H.~Uchida,
%``Finite modular subgroups for fermion mass matrices and baryon/lepton number violation,''
Phys. Lett. B \textbf{794}, 114-121 (2019)
doi:10.1016/j.physletb.2019.05.034
[arXiv:1812.11072 [hep-ph]].
%141 citations counted in INSPIRE as of 11 Oct 2023

%\cite{Novichkov:2018yse}
\bibitem{Novichkov:2018yse}
P.~P.~Novichkov, S.~T.~Petcov and M.~Tanimoto,
%``Trimaximal Neutrino Mixing from Modular A4 Invariance with Residual Symmetries,''
Phys. Lett. B \textbf{793}, 247-258 (2019)
doi:10.1016/j.physletb.2019.04.043
[arXiv:1812.11289 [hep-ph]].
%153 citations counted in INSPIRE as of 17 Oct 2023

%\cite{Kobayashi:2023zzc}
\bibitem{Kobayashi:2023zzc}
T.~Kobayashi and M.~Tanimoto,
%``Modular flavor symmetric models,''
[arXiv:2307.03384 [hep-ph]].
%11 citations counted in INSPIRE as of 17 Oct 2023

%\cite{Kobayashi:2019xvz}
\bibitem{Kobayashi:2019xvz}
T.~Kobayashi, Y.~Shimizu, K.~Takagi, M.~Tanimoto and T.~H.~Tatsuishi,
%``$A_4$ lepton flavor model and modulus stabilization from $S_4$ modular symmetry,''
Phys. Rev. D \textbf{100}, no.11, 115045 (2019)
[erratum: Phys. Rev. D \textbf{101}, no.3, 039904 (2020)]
doi:10.1103/PhysRevD.100.115045
[arXiv:1909.05139 [hep-ph]].
%106 citations counted in INSPIRE as of 17 Oct 2023

%\cite{Ishiguro:2020tmo}
\bibitem{Ishiguro:2020tmo}
K.~Ishiguro, T.~Kobayashi and H.~Otsuka,
%``Landscape of Modular Symmetric Flavor Models,''
JHEP \textbf{03}, 161 (2021)
doi:10.1007/JHEP03(2021)161
[arXiv:2011.09154 [hep-ph]].
%51 citations counted in INSPIRE as of 17 Oct 2023

%\cite{Abe:2020vmv}
\bibitem{Abe:2020vmv}
H.~Abe, T.~Kobayashi, S.~Uemura and J.~Yamamoto,
%``Loop Fayet-Iliopoulos terms in $T^2/Z_2$ models: Instability and moduli stabilization,''
Phys. Rev. D \textbf{102}, no.4, 045005 (2020)
doi:10.1103/PhysRevD.102.045005
[arXiv:2003.03512 [hep-th]].
%31 citations counted in INSPIRE as of 09 Oct 2023

%\cite{Novichkov:2022wvg}
\bibitem{Novichkov:2022wvg}
P.~P.~Novichkov, J.~T.~Penedo and S.~T.~Petcov,
%``Modular flavour symmetries and modulus stabilisation,''
JHEP \textbf{03}, 149 (2022)
doi:10.1007/JHEP03(2022)149
[arXiv:2201.02020 [hep-ph]].
%35 citations counted in INSPIRE as of 17 Oct 2023

%\cite{Ishiguro:2022pde}
\bibitem{Ishiguro:2022pde}
K.~Ishiguro, H.~Okada and H.~Otsuka,
%``Residual flavor symmetry breaking in the landscape of modular flavor models,''
JHEP \textbf{09}, 072 (2022)
doi:10.1007/JHEP09(2022)072
[arXiv:2206.04313 [hep-ph]].
%18 citations counted in INSPIRE as of 09 Oct 2023

%\cite{Knapp-Perez:2023nty}
\bibitem{Knapp-Perez:2023nty}
V.~Knapp-Perez, X.~G.~Liu, H.~P.~Nilles, S.~Ramos-Sanchez and M.~Ratz,
%``Matter matters in moduli fixing and modular flavor symmetries,''
Phys. Lett. B \textbf{844}, 138106 (2023)
doi:10.1016/j.physletb.2023.138106
[arXiv:2304.14437 [hep-th]].
%9 citations counted in INSPIRE as of 17 Oct 2023

%\cite{King:2023snq}
\bibitem{King:2023snq}
S.~F.~King and X.~Wang,
%``Modulus stabilisation in the multiple-modulus framework,''
[arXiv:2310.10369 [hep-ph]].
%0 citations counted in INSPIRE as of 18 Oct 2023

%\cite{Feruglio:2021dte}
\bibitem{Feruglio:2021dte}
F.~Feruglio, V.~Gherardi, A.~Romanino and A.~Titov,
%``Modular invariant dynamics and fermion mass hierarchies around $\tau = i$,''
JHEP \textbf{05}, 242 (2021)
doi:10.1007/JHEP05(2021)242
[arXiv:2101.08718 [hep-ph]].
%73 citations counted in INSPIRE as of 17 Oct 2023

%\cite{Novichkov:2021evw}
\bibitem{Novichkov:2021evw}
P.~P.~Novichkov, J.~T.~Penedo and S.~T.~Petcov,
%``Fermion mass hierarchies, large lepton mixing and residual modular symmetries,''
JHEP \textbf{04}, 206 (2021)
doi:10.1007/JHEP04(2021)206
[arXiv:2102.07488 [hep-ph]].
%62 citations counted in INSPIRE as of 17 Oct 2023

%\cite{Petcov:2022fjf}
\bibitem{Petcov:2022fjf}
S.~T.~Petcov and M.~Tanimoto,
%``$A_4$ modular flavour model of quark mass hierarchies close to the fixed point $\tau = \omega $,''
Eur. Phys. J. C \textbf{83}, no.7, 579 (2023)
doi:10.1140/epjc/s10052-023-11727-0
[arXiv:2212.13336 [hep-ph]].
%19 citations counted in INSPIRE as of 17 Oct 2023

%\cite{Kikuchi:2023cap}
\bibitem{Kikuchi:2023cap}
S.~Kikuchi, T.~Kobayashi, K.~Nasu, S.~Takada and H.~Uchida,
%``Quark hierarchical structures in modular symmetric flavor models at level 6,''
Phys. Rev. D \textbf{107}, no.5, 055014 (2023)
doi:10.1103/PhysRevD.107.055014
[arXiv:2301.03737 [hep-ph]].
%9 citations counted in INSPIRE as of 09 Oct 2023

%\cite{Abe:2023ilq}
\bibitem{Abe:2023ilq}
Y.~Abe, T.~Higaki, J.~Kawamura and T.~Kobayashi,
%``Quark masses and CKM hierarchies from $S_4^\prime$ modular flavor symmetry,''
[arXiv:2301.07439 [hep-ph]].
%11 citations counted in INSPIRE as of 17 Oct 2023

%\cite{Kikuchi:2023jap}
\bibitem{Kikuchi:2023jap}
S.~Kikuchi, T.~Kobayashi, K.~Nasu, S.~Takada and H.~Uchida,
%``Quark mass hierarchies and CP violation in A$_{4}$ \texttimes{} A$_{4}$ \texttimes{} A$_{4}$ modular symmetric flavor models,''
JHEP \textbf{07}, 134 (2023)
doi:10.1007/JHEP07(2023)134
[arXiv:2302.03326 [hep-ph]].
%11 citations counted in INSPIRE as of 17 Oct 2023

%\cite{Abe:2023qmr}
\bibitem{Abe:2023qmr}
Y.~Abe, T.~Higaki, J.~Kawamura and T.~Kobayashi,
%``Quark and lepton hierarchies from S4' modular flavor symmetry,''
Phys. Lett. B \textbf{842}, 137977 (2023)
doi:10.1016/j.physletb.2023.137977
[arXiv:2302.11183 [hep-ph]].
%8 citations counted in INSPIRE as of 17 Oct 2023

%\cite{Petcov:2023vws}
\bibitem{Petcov:2023vws}
S.~T.~Petcov and M.~Tanimoto,
%``A$_{4}$ modular flavour model of quark mass hierarchies close to the fixed point \ensuremath{\tau} = i\ensuremath{\infty},''
JHEP \textbf{08}, 086 (2023)
doi:10.1007/JHEP08(2023)086
[arXiv:2306.05730 [hep-ph]].
%8 citations counted in INSPIRE as of 17 Oct 2023

%\cite{Abe:2023dvr}
\bibitem{Abe:2023dvr}
Y.~Abe, T.~Higaki, J.~Kawamura and T.~Kobayashi,
%``Fermion hierarchies in SU(5) grand unification from $ {\Gamma}_6^{\prime } $ modular flavor symmetry,''
JHEP \textbf{08}, 097 (2023)
doi:10.1007/JHEP08(2023)097
[arXiv:2307.01419 [hep-ph]].
%5 citations counted in INSPIRE as of 17 Oct 2023

%\cite{deMedeirosVarzielas:2023crv}
\bibitem{deMedeirosVarzielas:2023crv}
I.~de Medeiros Varzielas, M.~Levy, J.~T.~Penedo and S.~T.~Petcov,
%``Quarks at the modular S$_{4}$ cusp,''
JHEP \textbf{09}, 196 (2023)
doi:10.1007/JHEP09(2023)196
[arXiv:2307.14410 [hep-ph]].
%3 citations counted in INSPIRE as of 17 Oct 2023

%\cite{Kobayashi:2017aeu}
\bibitem{Kobayashi:2017aeu}
T.~Kobayashi, N.~Omoto, H.~Otsuka and T.~H.~Tatsuishi,
%``Supersymmetry preserving and breaking degenerate vacua, and radiative moduli stabilization,''
Phys. Rev. D \textbf{96}, no.4, 046004 (2017)
doi:10.1103/PhysRevD.96.046004
[arXiv:1704.04875 [hep-th]].
%3 citations counted in INSPIRE as of 09 Oct 2023

%\cite{Kobayashi:2017zfd}
\bibitem{Kobayashi:2017zfd}
T.~Kobayashi, N.~Omoto, H.~Otsuka and T.~H.~Tatsuishi,
%``Radiative K\"ahler moduli stabilization,''
Phys. Rev. D \textbf{97}, no.10, 106006 (2018)
doi:10.1103/PhysRevD.97.106006
[arXiv:1711.10274 [hep-th]].
%6 citations counted in INSPIRE as of 09 Oct 2023

%\cite{deAdelhartToorop:2011re}
\bibitem{deAdelhartToorop:2011re}
R.~de Adelhart Toorop, F.~Feruglio and C.~Hagedorn,
%``Finite Modular Groups and Lepton Mixing,''
Nucl. Phys. B \textbf{858}, 437-467 (2012)
doi:10.1016/j.nuclphysb.2012.01.017
[arXiv:1112.1340 [hep-ph]].
%281 citations counted in INSPIRE as of 12 Oct 2023

%\cite{Altarelli:2010gt}
\bibitem{Altarelli:2010gt}
G.~Altarelli and F.~Feruglio,
%``Discrete Flavor Symmetries and Models of Neutrino Mixing,''
Rev. Mod. Phys. \textbf{82}, 2701-2729 (2010)
doi:10.1103/RevModPhys.82.2701
[arXiv:1002.0211 [hep-ph]].
%973 citations counted in INSPIRE as of 11 Oct 2023

%\cite{Ishimori:2010au}
\bibitem{Ishimori:2010au}
H.~Ishimori, T.~Kobayashi, H.~Ohki, Y.~Shimizu, H.~Okada and M.~Tanimoto,
%``Non-Abelian Discrete Symmetries in Particle Physics,''
Prog. Theor. Phys. Suppl. \textbf{183}, 1-163 (2010)
doi:10.1143/PTPS.183.1
[arXiv:1003.3552 [hep-th]].
%946 citations counted in INSPIRE as of 16 Oct 2023

%\cite{Kobayashi:2022moq}
\bibitem{Kobayashi:2022moq}
T.~Kobayashi, H.~Ohki, H.~Okada, Y.~Shimizu and M.~Tanimoto,
%``An Introduction to Non-Abelian Discrete Symmetries for Particle Physicists,''
2022,
ISBN 978-3-662-64678-6, 978-3-662-64679-3
doi:10.1007/978-3-662-64679-3
%19 citations counted in INSPIRE as of 09 Oct 2023

%\cite{Hernandez:2012ra}
\bibitem{Hernandez:2012ra}
D.~Hernandez and A.~Y.~Smirnov,
%``Lepton mixing and discrete symmetries,''
Phys. Rev. D \textbf{86}, 053014 (2012)
doi:10.1103/PhysRevD.86.053014
[arXiv:1204.0445 [hep-ph]].
%238 citations counted in INSPIRE as of 09 Oct 2023

%\cite{King:2013eh}
\bibitem{King:2013eh}
S.~F.~King and C.~Luhn,
%``Neutrino Mass and Mixing with Discrete Symmetry,''
Rept. Prog. Phys. \textbf{76}, 056201 (2013)
doi:10.1088/0034-4885/76/5/056201
[arXiv:1301.1340 [hep-ph]].
%802 citations counted in INSPIRE as of 17 Oct 2023

%\cite{King:2014nza}
\bibitem{King:2014nza}
S.~F.~King, A.~Merle, S.~Morisi, Y.~Shimizu and M.~Tanimoto,
%``Neutrino Mass and Mixing: from Theory to Experiment,''
New J. Phys. \textbf{16}, 045018 (2014)
doi:10.1088/1367-2630/16/4/045018
[arXiv:1402.4271 [hep-ph]].
%404 citations counted in INSPIRE as of 12 Oct 2023

%\cite{Tanimoto:2015nfa}
\bibitem{Tanimoto:2015nfa}
M.~Tanimoto,
%``Neutrinos and flavor symmetries,''
AIP Conf. Proc. \textbf{1666}, no.1, 120002 (2015)
doi:10.1063/1.4915578
%55 citations counted in INSPIRE as of 12 Oct 2023

%\cite{King:2017guk}
\bibitem{King:2017guk}
S.~F.~King,
%``Unified Models of Neutrinos, Flavour and CP Violation,''
Prog. Part. Nucl. Phys. \textbf{94}, 217-256 (2017)
doi:10.1016/j.ppnp.2017.01.003
[arXiv:1701.04413 [hep-ph]].
%198 citations counted in INSPIRE as of 09 Oct 2023

%\cite{Petcov:2017ggy}
\bibitem{Petcov:2017ggy}
S.~T.~Petcov,
%``Discrete Flavour Symmetries, Neutrino Mixing and Leptonic CP Violation,''
Eur. Phys. J. C \textbf{78}, no.9, 709 (2018)
doi:10.1140/epjc/s10052-018-6158-5
[arXiv:1711.10806 [hep-ph]].
%137 citations counted in INSPIRE as of 12 Oct 2023

%\cite{Ibanez:2012zz}
\bibitem{Ibanez:2012zz}
L.~E.~Ibanez and A.~M.~Uranga,
%``String theory and particle physics: An introduction to string phenomenology,''
Cambridge University Press, 2012,
ISBN 978-0-521-51752-2, 978-1-139-22742-1
%58 citations counted in INSPIRE as of 09 Oct 2023

%\cite{Coleman:1973jx}
\bibitem{Coleman:1973jx}
S.~R.~Coleman and E.~J.~Weinberg,
%``Radiative Corrections as the Origin of Spontaneous Symmetry Breaking,''
Phys. Rev. D \textbf{7}, 1888-1910 (1973)
doi:10.1103/PhysRevD.7.1888
%5032 citations counted in INSPIRE as of 19 Oct 2023

%\cite{Kikuchi:2022pkd}
\bibitem{Kikuchi:2022pkd}
S.~Kikuchi, T.~Kobayashi, K.~Nasu, H.~Otsuka, S.~Takada and H.~Uchida,
%``Modular symmetry of soft supersymmetry breaking terms,''
PTEP \textbf{2022}, no.12, 123B02 (2022)
doi:10.1093/ptep/ptac152
[arXiv:2203.14667 [hep-ph]].
%14 citations counted in INSPIRE as of 17 Oct 2023

%\cite{Dvali:2007wp}
\bibitem{Dvali:2007wp}
G.~Dvali and M.~Redi,
%``Black Hole Bound on the Number of Species and Quantum Gravity at LHC,''
Phys. Rev. D \textbf{77}, 045027 (2008)
doi:10.1103/PhysRevD.77.045027
[arXiv:0710.4344 [hep-th]].
%252 citations counted in INSPIRE as of 16 Oct 2023

%\cite{Kofman:2004yc}
\bibitem{Kofman:2004yc}
L.~Kofman, A.~D.~Linde, X.~Liu, A.~Maloney, L.~McAllister and E.~Silverstein,
%``Beauty is attractive: Moduli trapping at enhanced symmetry points,''
JHEP \textbf{05}, 030 (2004)
doi:10.1088/1126-6708/2004/05/030
[arXiv:hep-th/0403001 [hep-th]].
%293 citations counted in INSPIRE as of 12 Oct 2023

%\cite{Kikuchi:2023uqo}
\bibitem{Kikuchi:2023uqo}
S.~Kikuchi, T.~Kobayashi, K.~Nasu and Y.~Yamada,
%``Moduli trapping mechanism in modular flavor symmetric models,''
JHEP \textbf{08}, 081 (2023)
doi:10.1007/JHEP08(2023)081
[arXiv:2307.13230 [hep-ph]].
%1 citations counted in INSPIRE as of 09 Oct 2023

%\cite{Ishimori:2012zz}
\bibitem{Ishimori:2012zz}
H.~Ishimori, T.~Kobayashi, H.~Ohki, H.~Okada, Y.~Shimizu and M.~Tanimoto,
%``An introduction to non-Abelian discrete symmetries for particle physicists,''
Lect. Notes Phys. \textbf{858}, 1-227 (2012)
doi:10.1007/978-3-642-30805-5
%141 citations counted in INSPIRE as of 09 Oct 2023
